Don't Take the Easy Way Out: Ensemble Based Methods for Avoiding Known Dataset Biases

State-of-the-art models often make use of superficial patterns in the data that do not generalize well to out-of-domain or adversarial settings. For example, textual entailment models often learn that particular key words imply entailment, irrespective of context, and visual question answering models learn to predict prototypical answers, without considering evidence in the image. In this paper, we show that if we have prior knowledge of such biases, we can train a model to be more robust to domain shift. Our method has two stages: we (1) train a naive model that makes predictions exclusively based on dataset biases, and (2) train a robust model as part of an ensemble with the naive one in order to encourage it to focus on other patterns in the data that are more likely to generalize. Experiments on five datasets with out-of-domain test sets show significantly improved robustness in all settings, including a 12 point gain on a changing priors visual question answering dataset and a 9 point gain on an adversarial question answering test set.

==> sections/analysis.tex <==
\section{Learned-Mixin Analysis}
\label{sect:analysis}
In this section, we analyze the learned-mixin method in more detail to better understand why it improves upon the bias product method. 

\subsection{Synthetic Data}
% I thought this was interesting, but its taking up a lot of space....
It is illustrative to examine how models behave on the Dependent synthetic MNLI data. Recall that on this dataset a special indicator feature was added to each example, in addition to the bias feature, that was either 0 or 1, where 1 indicated the bias was randomized and 0 indicated that the bias was likely to agree with the label.

We observe that models trained in the bias-product ensemble learns to be \textit{anti}-biased in cases where the indicator is one. In particular, when the indicator is one the models assigns the class indicated by the bias an average of $22.5\%$ probability, where an unbaised model would have an average of $33\%$ since the data is approximately balanced.  
The root cause is a subtle training issue: if the indicator is 1, the model knows the bias is likely to be wrong, so it learns to subtract the value the bias-model will produce from its own output in order to cancel out the effect of the bias on the ensemble's output as a whole. This behaviour carries over to test-time and leads to errors.

The learned-mixin model avoids this issue, it assigns the class indicated by the bias an average of $34.5\%$ probability as expected. To explain why, we notice that the learned-mixed model learns to set $g(x_i)$ to $0.00 \pm 0.0001$ when the indicator is turned off, and to $1.91 \pm 0.285$ when the indicator is turned on. In short, it learns to turn off the bias when the indicator is one rather, than compensate for the bias's inaccuracy by changing the model's output, which prevents it falling prey to the same over-compensating effect.

\subsection{VQA-CP}

% \begin{table*}[]
%     \centering
%     \begin{tabular}{p{5cm}|l|c|c|c}
%         Question Type & Example & Factor & Factor (+H) & Bias Acc.\\ \hline
%         `Is...' yes/no questions & Is the dog sitting &  &  & \\
%         `Is...' non-yes/no questions & Is it dawn or dusk?  &  &  & \\
%         'How many...' questions about trees, sheep, or windows  & How many trees are there? & & & \\
%         `How many...' questions about dogs, giraffes, or cats  & How many cats are sitting down? & & & \\
%         % Contains `Or'  & Is it dawn or dusk? & $0.01 \pm 0.06$ & $1.62 \pm 0.79$ & \\
%         %   &  &  & & \\
%     \end{tabular}
%     \caption{Factors assigned to particular kinds of questions in VQA-CP. We show the factors as computed on the dev set, and the expected bias accuracy on those same kinds of questions on the train set. The model learns to down-weight the bias when is it known the bias will be inaccurate. For example, the bias tends to favour yes/no answers for questions that start with `is', 'does', `can', so it is weighted highly for yes/no questions that start with those phrases, but given little weight for exceptions. Likewise, the bias favours small numbers for questions that start with ``how many...", so model learns to put less weight on cases where the questions asks about things that tend to appear in larger groups.
%     }
%     \label{tab:my_label}
% \end{table*}

We similarly find that our VQA-CP learned-mixin model adjusts $g(x_i)$ when there is evidence in the example that indicates the bias might be inaccurate on VQA-CP. We suspect this helps remove bias for the same reason it does in the synthetic case: It prevents the model does not need to over-correct for errors in the bias when the it is known the bias will be inaccurate.

First, compute the expected bias accuracy (see the Appendix for details, and related scatter plots), and check to see how it correlated with the learned factors. We find a pearsonr correlation of 0.532, indicating a strong relation. We show some qualitative examples in Figure.


